Multimodal Reasoning with Multimodal Knowledge Graph

Multimodal reasoning with large language models (LLMs) often suffers from hallucinations and the presence of deficient or outdated knowledge within LLMs. Some approaches have sought to mitigate these issues by employing textual knowledge graphs, but their singular modality of knowledge limits comprehensive cross-modal understanding. In this paper, we propose the Multimodal Reasoning with Multimodal Knowledge Graph (MR-MKG) method, which leverages multimodal knowledge graphs (MMKGs) to learn rich and semantic knowledge across modalities, significantly enhancing the multimodal reasoning capabilities of LLMs. In particular, a relation graph attention network is utilized for encoding MMKGs and a cross-modal alignment module is designed for optimizing image-text alignment. A MMKG-grounded dataset is constructed to equip LLMs with initial expertise in multimodal reasoning through pretraining. Remarkably, MR-MKG achieves superior performance while training on only a small fraction of parameters, approximately 2.25% of the LLM's parameter size. Experimental results on multimodal question answering and multimodal analogy reasoning tasks demonstrate that our MR-MKG method outperforms previous state-of-the-art models.

==> table/table1.tex <==

\begin{table*}[t!]
\vspace{-0.1in}
\label{tab:main}
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule

\multirow{2}{*}{Method} &\multirow{2}{*}{\#T-Param} & \multicolumn{3}{c}{Subject} & \multicolumn{3}{c}{Context Modality} & \multicolumn{2}{c}{Grade} &  \multirow{2}{*}{Average} \\
     && NAT   & SOC   & LAN   & TXT   & IMG   & NO    & G1-6  & G7-12 &    \\ 
    \midrule

 Human~\cite{lu2022learn} &-&  90.23 & 84.97 & 87.48 & 89.60 & 87.50 & 88.10 & 91.59 & 82.42 & 88.40 \\
 GPT-3.5 (CoT)~\cite{lu2022learn} &-&  75.44 & 70.87 & 78.09 & 74.68 & 67.43 & 79.93 & 78.23 & 69.68 & 75.17 \\
 GPT-4~\cite{abs-2304-08485} &-& 84.06 & 73.45 & 87.36 & 81.87 & 70.75 & 90.73 & 84.69 & 79.10 & 82.69 \\ \midrule
UnifiedQA$_{Base}$~\cite{lu2022learn} &223M& {71.00} &  {76.04} &  {78.91} &  {66.42} &  {66.53} & {81.81} &  {77.06} & 68.82 &  {74.11} \\
UnifiedQA$_{Base}$(MM-CoT)~\cite{zhang2023multimodal} &223M&  87.52 & 77.17 & 85.82 & 87.88 & 82.90 & 86.83 & 84.65 & 85.37 & 84.91 \\
UnifiedQA$_{Large}$(MM-CoT)~\cite{zhang2023multimodal} & 738M&  \underline{\textbf{95.91}} & 82.00 & \underline{90.82} & \underline{95.26} & \underline{88.80} & \underline{92.89} & \underline{92.44} & 90.31 & \underline{91.68} \\
LLaVA~\cite{abs-2304-08485} &13B & 90.36 & \underline{\textbf{95.95}} & 88.00 & 89.49 & 88.00 & 90.66 & 90.93 & \underline{90.90} & 90.92 \\  \midrule
LLaMA-Adapter~\cite{zhang2023llama} &1.8M & 84.37 &  88.30  &  84.36  & 83.72 &  80.32 &  86.90 &  85.83 &  84.05 & 85.19 \\
LaVIN-7B~\cite{luo2023cheap} &3.8M & 89.25	&94.94 &	85.24&	88.51	&87.46	&88.08 &	90.16&	88.07 & 89.41\\
LaVIN-13B~\cite{luo2023cheap} & 5.4M &  89.88&	94.49	&89.82	&88.95&	87.61&	91.85&	91.45&	89.72& 90.83\\
\midrule

\textbf{MR-MKG(FLAN-T5-3B)} &77M & 90.67 &  85.38  &  86.45  & 90.96 &  87.46 &  87.39 &  90.27 &  85.23 & 88.47 \\
\textbf{MR-MKG(FLAN-T5-11B)} &248M &94.93	&90.1	&90.55	&94.53	&92.12	&92.2	&93.83	&90.9	&92.78\\
\textbf{MR-MKG(FLAN-UL2-19B)} & 248M &  95.74 &	90.33	&\textbf{92.00}	&\textbf{95.50} &\textbf{92.41}&	\textbf{93.31}&	\textbf{93.98}&	\textbf{93.01}& \textbf{93.63}\\


\bottomrule

\end{tabular}
}
\caption{Main results accuracy (\%) of ScienceQA \textit{test} set. \#T-Params = number of trainable parameters. Question classes: NAT = natural science, SOC = social science, LAN = language science, TXT = text context, IMG = image context, NO = no context, G1-6 = grades 1-6, G7-12 = grades 7-12. Segment 1: Zero- \& few-shot methods; Segment 2: SOTA and representative models; Segment 3: Parameter-efficient methods; Segment 4: Our MR-MKG results. %Results in \textbf{bold} are the best performance.
}
\vspace{-0.2in}
\end{table*}

==> table/table2.tex <==
\begin{table}[t]
    \centering
    \begin{center}
    \resizebox{0.475\textwidth}{!}{
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{lccccc}
    \toprule
    
    Method   & Hits@1 & Hits@3 & Hits@5 & Hits@10 & MRR \\
    \midrule

 IKRL~\cite{IKRL} & 0.266 & 0.294 & 0.301 & 0.310 & 0.283 \\
TransAE~\cite{TransAE}   & 0.261 & 0.285 & 0.289 & 0.293 & 0.276 \\
 RSME~\cite{RSME} & 0.266 & 0.298 & 0.307 & 0.311 & 0.285  \\ \midrule
 
MarT\_VisualBERT~\cite{VisualBERT}  & 0.261  & 0.292 & 0.308 & 0.321  & 0.284 \\
 MarT\_ViLT~\cite{ViLT} &0.245 & 0.275 & 0.287 & 0.303  & 0.266   \\
 MarT\_ViLBERT~\cite{ViLBERT} & 0.256  & 0.312 & 0.327  & 0.347  & 0.292 \\
 MarT\_FLAVA~\cite{FLAVA}  & 0.264 & 0.303 & 0.309 & 0.319 & 0.288  \\
 MarT\_MKGformer~\cite{MKGformer}  & \underline{0.301}  & \underline{0.367} & \underline{0.380} & \underline{0.408} & \underline{0.341} \\ \midrule
 
\textbf{Visual\_LLaMA-2 7B} &0.286 &0.373 &0.409 & 0.457 &0.347   \\
\textbf{MR-MKG(Visual\_LLaMA-2 7B)} &\textbf{0.405} &\textbf{0.465} &\textbf{0.497} &\textbf{0.531} &\textbf{0.449}    \\

    \bottomrule
    \end{tabular}
    }
    \end{center}
    \vspace{-0.15in}
    \caption{\small Main results of MARS \textit{test} set. Segment 1: multimodal knowledge graph embedding (MKGE) methods; Segment 2: multimodal pre-trained Transformer (MPT) methods; Segment 3: Our MR-MKG results. MarT represents that the model has been pre-trained on MarT. \textbf{Visual\_LLaMA} means that LLaMA is equipped with visual projection.}
    \label{tab:er}
    \vspace{-0.2in}
\end{table}

==> table/table3.tex <==

\begin{table*}[t!]
\vspace{-0.1in}
\label{tab:main}
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule

Settings    & NAT   & SOC   & LAN   & TXT   & IMG   & NO    & G1-6  & G7-12 & \multicolumn{1}{l}{Avg.} \\ \midrule

 Visual\_FLAN-T5-11B &88.45	&81.89	&84.09	&88.47	&86.51	&85.51	&86.75	&84.64	&86.08\tiny{{(+0.00)}}                  \\
+ KG                            &93.78	&88.64	&89.55	&93.35	&94.47	&91.08	&92.77	&89.65	&91.74\tiny{\textcolor{red}{(+5.66)}}                  \\
+ MMKG                            &94.23	&89.20	&90.00	&93.94	&91.77	&91.43	&93.39	&89.85	&92.21\tiny{\textcolor{red}{(+6.13)}}                  \\
+ Alignment                            & 94.40	&89.54	&90.09	&94.18	&91.77	&91.50	&93.32	&90.38	&92.36\tiny{\textcolor{red}{(+6.28)}}                  \\
+ Pre-training                            & 94.93	& 90.10	& 90.55	& 94.53	& 92.12	& 92.20	& 93.83	& 90.90	& 92.78\tiny{\textcolor{red}{(+6.70)}}                  \\
 


\bottomrule

\end{tabular}
}
\caption{Ablation study on ScienceQA \textit{test} set. Visual\_FLAN-T5 means that FLAN-T5 is equipped with visual projection. "KG" denotes textual knowledge graphs. "MMKG" indicates using MMKGs to replace KGs. }

\end{table*}

==> table/table4.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{center}
    \resizebox{0.475\textwidth}{!}{
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{lcc}
    
    \toprule

LLM   & Method & ScienceQA  \\
\midrule

\multirow{3}{*}{\textbf{FLAN-T5-11B}\hspace{0.3cm}}
 & Text-Only & 92.78 \\
 & Image-Only & 91.58  \\
 & Text + Image & 92.03  \\

 \bottomrule
    \end{tabular}
    }
    \end{center}
    \vspace{-0.15in}
    \caption{Average accuracy (\%) with different subgraph retrieve methods on ScienceQA \textit{test} set.}
    \label{tab:er}
\vspace{-0.25in}
\end{table}

==> table/table5.tex <==
\begin{table}[t]
    \centering
    \begin{center}
    \resizebox{0.475\textwidth}{!}{
    \renewcommand{\arraystretch}{1}

\begin{tabular}{lccc}
\toprule

Model &Design    & ScienceQA   & MARS \\ \midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}FLAN-T5-11B \\ /LLaMA2-7B\end{tabular}}\hspace{0.3cm}}
 &GNN &92.23	&39.1 \\

 & GAT &91.94	&39.6 \\
& RGAT &92.78	&40.5 \\

\bottomrule
    \end{tabular}
    }
    \end{center}
    \vspace{-0.15in}
    \caption{Results with different GNN  architectures on different tasks. In ScienceQA, the metric is Average accuracy (\%). In Task MARS, the metric is Hits@1(\%).}
    \label{tab:er}
\vspace{-0.25in}
\end{table}

